TensorOpt: Exploring the Tradeoffs in Distributed DNN Training with Auto-Parallelism

A good parallelization strategy can significantly improve the efficiency or reduce the cost for the distributed training of deep neural networks (DNNs). Recently, several methods have been proposed to find efficient parallelization strategies but they all optimize a single objective (e.g., execution time, memory consumption) and produce only one strategy. We propose FT, an efficient algorithm that searches for an optimal set of parallelization strategies to allow the trade-off among different objectives. FT can adapt to different scenarios by minimizing the memory consumption when the number of devices is limited and fully utilize additional resources to reduce the execution time. For popular DNN models (e.g., vision, language), an in-depth analysis is conducted to understand the trade-offs among different objectives and their influence on the parallelization strategies. We also develop a user-friendly system, called TensorOpt, which allows users to run their distributed DNN training jobs without caring the details of parallelization strategies. Experimental results show that FT runs efficiently and provides accurate estimation of runtime costs, and TensorOpt is more flexible in adapting to resource availability compared with existing frameworks.

==> TO_algorithm.tex <==
\section{The Frontier Tracking Algorithm}\label{sec:alg}

In this section, we present the Frontier Tracking (FT) algorithm



\subsection{Algorithm Description}\label{subsec:algorithm description}



For simplicity of discussion, we only present the FT algorithm for finding the frontier of execution time $t(S, \mathcal{G}, \mathcal{D})$ and memory consumption $m(S, \mathcal{G}, \mathcal{D})$. Generalizing the algorithm to track the frontier for any pair of costs (e.g., memory consumption and network communication) should be straightforward. We first give the formal definition of \textit{cost frontier} as follows.



%\begin{algorithm}
%	\caption{F-Opt}
%	\label{alg:F-Opt}
%	\begin{algorithmic}[1]
%		\STATE {\bfseries Input:} Computation graph $\mathcal{G}$, device graph $\mathcal{D}$
%		\STATE {\bfseries Output:} All parallelization strategies on the cost frontier of execution time and memory consumption    
%		\STATE Initialize the cost frontier for operators and edges in  $\mathcal{G}$
%		\WHILE{true}
%		\STATE Mark nodes on the linear graph
%		\IF {Elimination($\mathcal{G}$)}
%		\STATE continue
%		\ENDIF
%		\STATE break
%		\ENDWHILE
%		\STATE Apply \textit{linear DP} on the final graph and generate the strategies on the cost frontier
%		\STATE Unroll the linear DP
%		\STATE Unroll the elimination
%	\end{algorithmic}
%\end{algorithm} 

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.60\columnwidth]{./figure/frontier-crop.pdf}
  \caption{An illustration of cost frontier}
  \label{fig:cost frontier}
\end{figure}


%\begin{cost frontier}\label{def:frontier}
%	Let $\mathcal{C}\!=\!\{(m_1, t_1), (m_2, t_2),\cdots, (m_k, t_k)\}$ be a set of cost tuples, its frontier $\mathcal{F}$ is the smallest subset of $\mathcal{C}$ that satisfies for any $(m_j, t_j)\in \mathcal{C}-\mathcal{F}$, there exists a $(m_i, t_i)\in \mathcal{F}$ with $m_i\le m_j, t_i\le t_j$.         
%\end{cost frontier}

\begin{cost frontier}\label{def:frontier}
%Let $\mathcal{C}\!=\!\{(S_1, m_1, t_1), (S_2, m_2, t_2),\cdots, (S_K,\\ m_K, t_K)\}$ be a set of (partial) parallelization strategy tuples, where $S_k$ is a (partial) parallelization strategy, $m_k$ and $t_k$ are two non-negative costs of $S_k$,  for $1\le k \le K$. The cost frontier of $\mathcal{C}$ is its smallest subset $\mathcal{F}$ such that, for any strategy tuple $(S_p, m_p, t_p)\in \mathcal{C}-\mathcal{F}$, there exists a strategy tuple $(S_k, m_k, t_k)\in \mathcal{F}$ where $m_k\le m_p$ and $t_k\le t_p$.        
Let $\mathcal{C}\!=\!\{(S_1, m_1, t_1), (S_2, m_2, t_2),\cdots, (S_K,\\ m_K, t_K)\}$ be a set of (partial) parallelization strategy tuples, where $S_k$ is a (partial) parallelization strategy, $m_k$ and $t_k$ are two non-negative costs of $S_k$,  for $1\le k \le K$. The cost frontier of $\mathcal{C}$ is a subset $\mathcal{F}$ of $\mathcal{C}$ such that, for any strategy tuple $(S_p, m_p, t_p)\in \mathcal{C}$, there exists a strategy tuple $(S_k, m_k, t_k)\in \mathcal{F}$ where $m_k\le m_p$ and $t_k\le t_p$.
\end{cost frontier}

We provide an illustration of the cost frontier of some random points (by plotting only the two costs) in Figure~\ref{fig:cost frontier}. According to Definition~\ref{def:frontier}, for a strategy that is not in the cost frontier, we can find some strategy in the frontier that can reduce at least one of the two costs without increasing the other. Therefore, it suffices to find all parallelization strategies in the frontier of $t(S, \mathcal{G}, \mathcal{D})$ and $m(S, \mathcal{G}, \mathcal{D})$. Users can choose a parallelization strategy according to the situation (e.g., the amount of available memory) once the frontier is found. With a slight abuse of the notations, we use $\mathcal{F}(o_i,s_i^k)$ to denote the tuple $(s_i^k, m(o_i, s_i^k), t(o_i, s_i^k))$ (i.e., the operator costs in Eq.~\eqref{equ:operator cost}), which is the cost frontier for operator $o_i$ when it selects $s_i^k$ as the parallelization configuration. Similarly, $\mathcal{F}(e_{ij},s_i^k,s_j^p)$ denotes the tuple $([s_i^k,s_j^p], m(e_{ij},s_i^k,s_j^p),t(e_{ij},s_i^k,s_j^p))$ (i.e., the edge costs in Eq.~\eqref{equ:operator cost}), which is the cost frontier for edge $e_{ij}$ when operator $o_i$ and $o_j$ use parallelization configuration $s_i^k$ and $s_j^p$, respectively. Although both $\mathcal{F}(o_i,s_i^k)$ and $\mathcal{F}(e_{ij},s_i^k,s_j^p)$ have a cardinality of 1 initially, their size may change when the FT algorithm updates them.

%The cost frontier of a set can be identified using Algorithm~\ref{alg:frontier}, , in which $\mathcal{C}_m[i]$ is the $i^{\textsubscript{th}}$ tuple in $\mathcal{C}_m$ and $r_t(\mathcal{C}_m[i])$ in the position of tuple $\mathcal{C}_m[i]$ in $\mathcal{C}_t$. 

Given a set of strategies, $\mathcal{C}$, it is simple to obtain the cost frontier of $\mathcal{C}$ as described in Algorithm~\ref{alg:frontier}. In Algorithm~\ref{alg:frontier}, $\mathcal{C}_m$ and $\mathcal{C}_t$ are the two sets obtained by sorting $\mathcal{C}$ according to memory and time consumption, respectively, and $\mathcal{C}_m[i]$ is the $i^{\textsubscript{th}}$ tuple in $\mathcal{C}_m$ and $r_t(\mathcal{C}_m[i])$ in the position of the tuple $\mathcal{C}_m[i]$ in $\mathcal{C}_t$. \textbf{[james: pls add a brief explanation of the algorithm.]}



\begin{algorithm}
  \caption{Frontier Finding}
  \label{alg:frontier}
  \begin{algorithmic}[1]
    \STATE {\bfseries Input:} A set $\mathcal{C}$ containing $K$ strategy tuples
    \STATE {\bfseries Output:} The cost frontier $\mathcal{F}$ of $\mathcal{C}$
    \STATE Sort tuples in $\mathcal{C}$ in ascending order of memory consumption and denote the result as $\mathcal{C}_m$
    \STATE Sort tuples in $\mathcal{C}$ in ascending order of time consumption and denote the result as $\mathcal{C}_t$
    \STATE Initialize $\mathcal{F}=\emptyset$, $v=K+1$
    \FOR{\texttt{$i = 1$ to $K$}}
    \IF{$r_t(\mathcal{C}_m[i])<v$}
    \STATE $\mathcal{F}=\mathcal{F}\cup \mathcal{C}_m[i]$ and $v=r_t(\mathcal{C}_m[i])$
    \ENDIF
    \ENDFOR
    \STATE Return $\mathcal{F}$
  \end{algorithmic}
\end{algorithm}



%With a slight abuse of notation, we use $\mathcal{F}(o_i,s_i^k)$ to denote the tuple $(s_i^k, m(o_i, s_i^k), t(o_i, s_i^k))$, in which $m(o_i, s_i^p)$ and $t(o_i, s_i^p)$ are defined in eq.~\ref{equ:operator cost}. Similarly, $\mathcal{F}(e_{i-1}^i,s_{i-1}^k,s_i^p)$ denote the tuple $([s_{i-1}^k,s_i^p], m(e^i_j,s_{i-1}^k,s_i^p),t(e^i_j,s_{i-1}^k,s_i^p))$ as defined in eq.~\ref{equ:edge cost}.          

%\textbf{[james: need a general intro here, talk about the connection between Alg 1 and Alg 2]}

We now present the FT algorithm, as outlined in Algorithm~\ref{alg:FT}. We first introduce some~\textit{basic operations}, which FT uses to manipulates cost frontiers. Given two cost frontiers (or two sets of strategy tuples),
\[
  \begin{aligned}
    \mathcal{F}  & =\{(S_1, m_1, t_1), (S_2, m_2, t_2),...,(S_K, m_K,t_K)\},                   \\
    \mathcal{F}' & =\{(S_1', m_1', t_1'), (S_2', m_2', t_2'),...,(S_{K'}', m'_{K'},t'_{K'})\}.
  \end{aligned}
\]


\begin{description}
  \item[$\bullet$]\textbf{Product}, which is the Cartesian product of two frontiers:
        $$\mathcal{F} \otimes \mathcal{F}' = \cup_{1\le k \le K, 1\le p \le K'}\left\{\big([S_k, S_p'], m_k+m_p', t_k+t_p'\big)\right\}.$$
  \item[$\bullet$]\textbf{Union}, which is the union of two frontiers:
        $$ \mathcal{F} \cup \mathcal{F}' = \cup_{1\le k \le K}\{(S_k, m_k,t_k)\}\,\,\cup \,\, \cup_{1\le p \le K'}\{(S_p', m_p',t_p')\}.$$
  \item[$\bullet$]\textbf{Reduce}, which is Algorithm~\ref{alg:frontier}, i.e., $\mathcal{F}=\text{reduce} (\mathcal{C})$. As the result of \textit{product} and \textit{union} may no longer be a frontier, we assume that \textit{reduce} is always applied after the two operations.%\footnote{We omit the \textit{reduce} for conciseness in the rest of the paper.}.           
\end{description}

Intuitively, \textit{product} constructs composite parallelization strategies by enumerating all possible combinations of $S$ and $S'$, and the costs of $S$ and $S'$ are summed up in the product. The operation \textit{union} places the tuples from $\mathcal{F}$ and $\mathcal{F}'$ into a single set.

%FT is based on dynamic programming (DP). 

Algorithm~\ref{alg:FT} first initializes the cost for each operator (or edge) in $\mathcal{G}$ by enumerating all possible parallelization configurations of the operator (or the two operators associated with the edge). Then the algorithm conducts elimination to simplify the computation graph $\mathcal{G}$ (Lines~4-11), finds the cost frontier on the simplified graph $\mathcal{G}'$ (Line~12), and finally unrolls the simplified graph to reconstruct the parallelization strategies in the cost frontier for the entire computation graph $\mathcal{G}$  (Lines~13-14).

The FT algorithm is based on dynamic programming (DP), but it has fundamental differences from the DP algorithm in OptCNN~\cite{OptCNN}. First, it simplifies the computation graph into a linear graph instead of two nodes (as in OptCNN) and applies linear DP (LDP) on the linear graph, as illustrated in Figure~\ref{fig:linear graph}. We will show that using LDP significantly reduces the complexity. Second, FT manages the cost frontier of a pair of costs (e.g., execution time and memory consumption) instead of only execution time, which requires a redesign of the elimination procedures. Finally, FT conducts more types of elimination to adapt to different types of networks (e.g., OptCNN~\cite{OptCNN} does not apply to BERT~\cite{bert}) and reduce the complexity.

We first present the details of LDP on the linear graph, the elimination procedures, and unrolling LDP and elimination, as follows.


\begin{algorithm}
  \caption{Frontier Tracking (FT)}
  \label{alg:FT}
  \begin{algorithmic}[1]
    \STATE {\bfseries Input:} Computation graph $\mathcal{G}$, device graph $\mathcal{D}$
    \STATE {\bfseries Output:} All parallelization strategies in the cost frontier of execution time and memory consumption
    \STATE Initialize all valid parallelization configurations and their costs for the operators and edges in $\mathcal{G}$
    \WHILE{true}
    \STATE Mark nodes on the linear graph
    \IF {not TryExactEliminate($\mathcal{G}$)}
    \IF {not TryHeuristicEliminate($\mathcal{G}$)}
    \STATE break
    \ENDIF
    \ENDIF
    % \IF {an unmarked node or some edges can be eliminated}
    % \STATE Eliminate($\mathcal{G}$)
    % \STATE continue
    % \ENDIF
    % \STATE break
    \ENDWHILE
    \STATE Apply LDP in Algorithm~\ref{alg:Linear-dp} on the simplified graph $\mathcal{G'}$ and generate strategies on the cost frontier
    \STATE Unroll the LDP
    \STATE Unroll the elimination
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}
  \caption{Linear Dynamic Programming (LDP)}
  \label{alg:Linear-dp}
  \begin{algorithmic}[1]
    \STATE {\bfseries Input:} A linear computation graph $\mathcal{G'}$ and its size $n$
    \STATE {\bfseries Output:} All parallelization strategies in the cost frontier of execution time and memory consumption
    \STATE $\mathcal{G}'(o_1, s^k_1) = \mathcal{F}(o_1, s^k_1)$ for $s^k_1 \in \mathcal{S}_1$
    \FOR{\texttt{$i = 2$ to $n$}}
    \FOR{\texttt{$s^p_i \in \mathcal{S}_i$}}
    \STATE $\mathcal{G}'(o_i, s^p_i) = \cup_{s_{i-1}^k \in \mathcal{S}_{i-1} }\{\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)\otimes \mathcal{G}'(o_{i-1},s_{i-1}^k)\otimes \mathcal{F}(o_i,s_i^p)$\}
    \ENDFOR
    \ENDFOR
    \STATE $\mathcal{F}_o = reduce(\cup_{s_n^k\in\mathcal{S}_n}\mathcal{G}'(n,s_n^k))$
    \STATE Return $\mathcal{F}_o$
  \end{algorithmic}
\end{algorithm}


%\textit{provide an illustration of linear graph; or two compare the enlimination goal of optcnn and }



\textbf{Linear Dynamic Programming}. We found that if the computation graph $\mathcal{G}$ has a linear structure (as shown in Figure~\ref{fig:linear graph}), its cost frontier can be found much more efficiently than conducting elimination in OptCNN~\cite{OptCNN}. Moreover, popular DNN models can be easily organized into a linear structure. For example, if we treat each residual block as a group for ResNet~\cite{}, then the groups form a linear structure. For Transformer~\cite{}, each transformer block can also be regarded as a group and the transformers form a linear structure.

Therefore, different from OptCNN, which tries to eliminate as many operators and edges as possible, FT conducts elimination such that the resultant graph $\mathcal{G}'$ has a linear structure. We use a simple heuristic for this purpose in Algorithm~\ref{alg:FT} when choosing the nodes and edges to eliminate. Before elimination starts, we mark the first operator~\footnote{According to topological order, ties are broken randomly.} in the computation graph $\mathcal{G}$. During elimination, we do not eliminate the marked operators, and checks if the last operator we marked has only one output operator. If so, we mark that output operator as it is also on a linear structure. After obtaining a linear structure, Algorithm~\ref{alg:Linear-dp} (LDP) is used to compute the cost frontier.

In Algorithm~\ref{alg:Linear-dp}, we assume that the cost frontiers of the operators and edges (i.e., $\mathcal{F}(o_i,s_i^k)$ and $\mathcal{F}(e_{ij},s_i^k,s_j^p)$) in the linear graph $\mathcal{G}'$ are properly initialized (the initialization method will be introduced shortly in the \textit{elimination} part).  The algorithm computes the cost frontier of $\mathcal{G}'$ from the operator that receives the initial input (numbered as $o_1$) to the operator that generates the final model output (numbered as $o_n$). For the first operator $o_1$, we initialize its cumulative cost frontier $\mathcal{G}'(o_1, s^k_1)$ as $\mathcal{F}(o_1,s^k_1)$. For the $i^{th}$ operator, we use the product of $\mathcal{G}'(o_{i-1}, s^k_{i-1})$, the frontier $\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)$ of edge $e_{(i-1)i}$, and $\mathcal{F}(o_i, s_i^p)$ to update $\mathcal{G}(o_i, s_i^p)$. Therefore, $\cup_{s_i^p\in\mathcal{S}_i}\mathcal{G}(o_i, s_i^p)$ represent the \textit{cumulative cost frontier} from operator $o_1$ to $o_i$.\textbf{ [james: cumulative cost frontier needs to be first intuitively introduced of its meaning and purpose.]}




%, which is the cost frontier when using parallelization configuration $s^k_1$ for operator $o_1$ (can contain only a single element)








As we will show in Section~\ref{subsec:complexity analysis}, for a linear graph $\mathcal{G}'$ with $n$ operators and each operator has at most $K$ feasible parallelization configurations, the complexity of LDP in Algorithm~\ref{alg:Linear-dp} is $O(n^2K^2\log(K)(\log(n)+\log(K)))$. In contrast, using OptCNN style node elimination to track the cost frontier has a complexity of $O(n^2K^3\log(K)(\log(n)+\log(K)))$, which is much more costly than LDP due to the large value of $K$.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.7\columnwidth]{./figure/ldp-crop.pdf}
  \caption{An illustration of the difference between FT and OptCNN}
  \label{fig:linear graph}
\end{figure}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=1.6\columnwidth]{./figure/elimination-crop.pdf}
  \caption{An illustration of different types of elimination in FT}
  \label{fig:elimination}
\end{figure*}

\vspace{1mm}
\textbf{Elimination.} FT conducts four types of elimination: \textit{node elimination}, \textit{edge elimination}, \textit{branch elimination}, and \textit{heuristic elimination}. The first three preserve the exact cost frontier, while heuristic elimination significantly reduces the complexity with only a small loss in accuracy. Compared with the two types of elimination (i.e., node and edge elimination) in OptCNN, more types of elimination enable FT to adapt to a more diverse set of DNN models (e.g., RNN).  Moreover, for each type of elimination, FT maintains the cost frontier instead of a single cost. We provide an illustration of the different types of elimination in Figure~\ref{fig:elimination} and explain them as follows.
\vspace{1mm}

\textit{Node Elimination}. FT conducts node elimination when an operator has only one input operator and one output operator. As shown in Figure~\ref{fig:elimination}(a), $e_{hi}$, $o_i$ and $e_{ij}$ are replaced by a single edge $e_{hj}$ in node elimination. The cost frontier of $e_{hj}$ is deduced as follows

%$h, i,j$ $k,p,w$
\begin{equation}\label{equ:node}
  \begin{aligned}
    \mathcal{F}(e_{hj}, s_h^w, s_j^p) & = \cup_{s_i^k\in\mathcal{S}_i}\{\mathcal{F}(e_{hi}, s_h^w, s_i^k) \otimes \mathcal{F}(o_i, s_i^k) \\
                                      & \quad \quad \quad \quad \otimes \mathcal{F}(e_{ij}, s_i^k, s_j^p)\}.
  \end{aligned}
\end{equation}

Under each combination of the parallelization configurations of operators $o_h$ and $o_j$, $o_i$ is eliminated by summing its operator cost to the costs on edge $e_{hi}$ and $e_{ij}$. Note that we apply~\textit{reduce} to the result of Eq.~\eqref{equ:node} to ensure that $\mathcal{F}(e_{hj}, s_h^w, s_j^p)$ is a frontier, which reduces the size of $\mathcal{F}(e_{hj}, s_h^w, s_j^p)$ and the complexity of subsequent operations. For each tuple in the frontier $\mathcal{F}(e_{hj}, s_h^w, s_j^p)$, FT records which parallelization configuration $o_i$ (i.e., $s_i^k$) takes to produce it in order to provide information for unrolling the elimination. When the computation graph $\mathcal{G}$ is a linear graph, we can also apply node elimination to simplify the graph to only 2 nodes to track the cost frontier, which is similar to the DP algorithm in OptCNN. We call this method \textit{FT-Elimination} and compare its complexity with FT-LDP in Section~\ref{subsec:complexity analysis}.


%As the result may contain points that do not belong to the cost frontier, we use the reduce operation to remove them.

\vspace{1mm}
\textit{Edge Elimination}. FT conducts edge elimination when there are multiple edges connecting the same pair of operators. Denote the edges as $(e_{ij}^1, e_{ij}^2, ...,e_{ij}^V)$, these edges are merged into a single edge $e_{ij}$, as illustrated in Figure~\ref{fig:elimination}(b). The cost frontier of the new edge is calculated as follows
\begin{equation}
  \mathcal{F}(e_{ij}, s_i^k, s_j^p) = \otimes_{1\leq v \le V} \mathcal{F}(e_{ij}^v, s_i^k, s_j^k).
\end{equation}
Under the same parallelization configuration of the up-stream operator $o_i$ and down-stream operator $o_j$, the costs of the merged edges are added together for edge elimination. As node and edge elimination cannot reduce some complex computation graphs (e.g., BERT~\cite{bert}) to simple structures, we introduce \textit{branch elimination and heuristic elimination}, which OptCNN does not have.
%Then the results that do not belong to the frontier are removed.  

\vspace{1mm}
\textit{Branch Elimination}. FT conducts branch elimination when an operator has multiple input operators and these operators cannot be eliminated by node or edge elimination. An example is shown in Figure~\ref{fig:elimination}(c), in which operator $o_h$ receives inputs from operators $o_i$ and $o_j$, and $o_i$ and $o_j$ cannot be eliminated because they are not connected by an edge. Branch elimination removes either $o_i$ or $o_j$ by merging it into $o_h$. If $o_i$ is merged, the cost frontier of $o_h$ is updated as follows
\begin{equation}
  \begin{aligned}
    \mathcal{F}(o_h, \tilde{s}_k^w) = & \cup_{s_i^k\in\mathcal{S}_i}\{\mathcal{F}(o_h, s_h^p) \otimes \mathcal{F}(o_i, s_i^k) \\
                                      & \otimes \mathcal{F}(e_{ih}, s_i^k, s_h^p)\},
  \end{aligned}
\end{equation}
where $\tilde{s}_k^w=(s_h^p,s_i^k)$ is the concatenation of the parallelization configuration of $o_i$ and $o_k$, and the costs of operator $o_i$ and edge $e_{ih}$ are added to the cost of operator $o_h$.


%\begin{branch enlimination}
%	Node elimination, edge elimination and branch elimination correctly preserves the cost frontier of the original computation graph $\mathcal{G}$.
%\end{branch enlimination} 

%The proof can be found in the supplementary material.
\vspace{1mm}
\textit{Heuristic Elimination}. FT conducts heuristic elimination when the three types of elimination introduced before cannot be applied, which may happen for models such as Bert~\cite{bert}. In Bert, the attention mask is used by all the transformer layer. An example is shown in Figure~\ref{fig:elimination} (d), in which the computation graph cannot be simplified with other types of elimination. In this case, heuristic elimination decides the parallelization configuration for an operator $o_i$, and removes $o_i$ along with all its out-going edges. We use multiple heuristics to choose a parallelization configuration for $o_i$, e.g., minimizing the memory consumption of $o_i$ or a weighted combination of different objectives. After removing $o_i$ by selecting parallelization configuration $s_i^k$, an operator $o_j$ that takes input from $o_i$ updates its frontier as follows
\begin{equation}
  \mathcal{F}(o_j, s_j^p) = \mathcal{F}(o_j, s_j^p) \otimes \mathcal{F}(e_{ij}, s_i^k, s_j^p),
\end{equation}
which adds the cost of edge $e_{ij}$ to operator $o_j$. Note that heuristic elimination does not guarantee to preserve the cost frontier. However, we found that it significantly reduces the running time of FT with only marginal loss in accuracy. This is because we usually conduct heuristic elimination for only a very small number of times. For example, heuristic elimination only needs to be used once for BERT.

\vspace{1mm}
\textbf{Unrolling LDP and elimination.} FT unrolls the strategy tuples in the final cost frontier $\mathcal{F}_o$ produced by LDP in Algorithm~\ref{alg:Linear-dp} to reconstruct the parallelization strategies for the entire computation graph $\mathcal{G}$. To provide information for unrolling, in each step of LDP and for each strategy tuple in $\mathcal{G}'(o_i, s^p_i)$, FT records the parallelization configuration of $o_{i-1}$ (i.e., $s_{i-1}^k$) and the strategy tuple in $\mathcal{G}'(o_{i-1},s_{i-1}^k)$ that produces it. Therefore, the final strategy tuples are unrolled by tracing back each step of LDP recursively. For unrolling elimination, FT records the parallelization configuration taken by the eliminated operator for each tuple in the cost frontier $\mathcal{F}$ produced by the elimination. Once we know the selected partial strategy in $\mathcal{F}$, the parallelization configuration of the eliminated operator can be reconstructed.



\vspace{1mm}
\textbf{Optimizations for efficiency.}

The execution of FT can be parallelize naturally. In LDP, the cumulative cost frontier $\mathcal{G}'(o_i)$ of different strategies can be computed independently since they only read from $\mathcal{G}'(o_{i-1})$. In the elimination, for the cost frontier $\mathcal{F}(e_{hj}, s_h^w, s_j^p)$, the computation of different $s_h^w$ and $s_j^p$ are also independent. During the elimination or linear dp, we spawn multiple threads for accleration.

\vspace{1mm}
\textbf{Optimizations for accuracy.} The memory consumption and execution time of the operators (under different parallelization configurations) are easy to predict~\cite{OptCNN,FlexFlow}. Thus the accuracy of the overall cost estimation provided by FT strongly depends on the quality of communication time (i.e., $t_x(e_{ij}, s_i^k, s_j^p)$ and $t_s(o_i, s_i^k)$ in Section~\ref{sec:related}) estimation. FlexFlow and OptCNN calculate the communication time using the amount of data to be transferred divided by the speed of the network connection between the devices. We found that this estimation method can lead to very large error for several reasons. First, latency could dominate the communication time when transferring small tensors between GPUs. Second, as they use send-recv for communication, several send-recv operations could be executed by different devices simultaneously and these operations will contend for the PCIE or IB bandwidth, which makes communication time difficult to estimate. We use collective operations for all the network communication, which avoids possible contention. As introduced in Section~\ref{sec:related}, we profile the communication time under different message sizes and device topologies, and fit xxx model to predict the communication time.

\vspace{1mm}
We observe that a parallel strategy for an operator divides the devices into disjoint groups and the communication take place each group independently. For each group the amount of data needed to tranfer are the same. Different groups may contend for the same physical connection bandwidth like PCIe or IB. Therefore, we use profiled bandwidth for each device paratition scheme to predict the network communication time. Specifically, for a device partition scheme, we profile the bandwidth for collective operation for the data size $ 2 ^ i$, where $ 0 \leq i < P$. $P$ is a sufficient large integer to cover all the data size. When we predict the network time for data size $k$, we find $i$ satisfying $2 ^i \leq k < 2 ^ {i + 1}$ and use the interpolation of bandwidth at $2 ^ i$ and $2 ^ {i + 1}$ to predict the running time. From the experiment, we show that the prediction error is only about $6-7\% $.


\textit{more details about the machine learning model}




\subsection{Complexity Analysis}\label{subsec:complexity analysis}


In this part, we analyze the complexity of FT in Algorithm~\ref{alg:FT} and LDP in Algorithm~\ref{alg:Linear-dp}, and compare their complexity with that of FT-Elimination.

\begin{frontier complexity}\label{lemma:frontier complexity}
For a set $\mathcal{C}$ containing $K$ (partial) parallelization strategy tuples, its cost frontier can be obtained with a complexity of $O(K\log(K))$ using Algorithm~\ref{alg:frontier}.
\end{frontier complexity}

The proof of Lemma~\ref{lemma:frontier complexity} is straightforward as the complexity of Algorithm~\ref{alg:frontier} is dominated by sorting the $K$ tuples.

\begin{random tuple}\label{assup:random tuple}
For a set $\mathcal{C}$ containing $K$ strategy tuples, let $r_m(S_p, m_p, t_p)$ and $r_t(S_p, m_p, t_p)$ be the rank of tuple $(S_p, m_p, t_p)$ when sorting $\mathcal{C}$ in ascending order of memory and time consumption, respectively. $\mathcal{C}$ is said to have random order if $\mathcal{P}[r_m(S_p, m_p, t_p)=k]=\frac{1}{K}$ and $\mathcal{P}[r_t(S_p, m_p, t_p)=h]=\frac{1}{K}$ for $1 \le p, k, h \le K$, and $r_m(S_p, m_p, t_p)$ and $r_t(S_p, m_p,\\ t_p)$ are independent.
\end{random tuple}

In the following analysis, we always assume that a set $\mathcal{C}$ has  random order solving its cost frontier.

\textit{why this assumption is not very restrictive?}

\begin{random size}\label{lemma:random size}
For tuple set $\mathcal{C}$ having random order and containing $K$ tuples, the expected size of its cost frontier $\mathcal{F}$ is $\log(K)$.
\end{random size}


\begin{proof}
  Denote the expected size of $\mathcal{F}$ as $f(K)$, which is a function of the cardinality of the tuple set $\mathcal{C}$. Consider the tuple having the minimum time consumption in $\mathcal{C}$ (denoted as $S_p$), it is obvious that $S_p\in \mathcal{F}$ and tuples having larger memory consumption than $S_p$ do not belong to $\mathcal{F}$ (by the definition of cost frontier). The cost frontier of the tuples having smaller memory consumption than $S_p$ also belongs to $\mathcal{F}$, and the number of these tuples follows a discrete uniform distribution on $\{0,1,\cdots, K-1\}$ due to the random order assumption. Therefore, we can get the following recursive function,
  $$ f(K) = \sum_{k=1}^{K} \frac{f(k-1)}{K}  + 1.$$
  Solving the recursive function, we have $f(K) = \sum_{k=1}^{K} \frac{1}{k} = O(\log(K))$.
\end{proof}

We analyze the complexity of FT-LDP and FT-Elimination for frontier tracking \textit{when the computation graph $\mathcal{G}$ is a linear graph}. In this case, both $\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)$ and $\mathcal{F}(o_i,s_i^p)$ has a cardinality of 1. For more complicated graphs, FT-Elimination may not work while for FT-LDP the cardinalities of $\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)$ and $\mathcal{F}(o_i,s_i^p)$ depend on the elimination operations (which in turn depends on the structure of the computation graph). We also give the one-step complexity of FT-LDP and FT-Elimination when the cardinality of $\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)$ is not 1.

\begin{one step complexity}\label{theorem:one step complexity}
For FT-LDP in Algorithm~\ref{alg:Linear-dp}, assume that operators $o_{i-1}$ and $o_i$ both have $K$ parallelization configurations, the cumulative cost frontier $\mathcal{G}'(o_{i-1},s_{i-1}^k)$ of $o_{i-1}$  has a cardinality of $a$, and the edge cost frontier $\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)$ has a cardinality of $b$. The complexity of solving the cumulative cost frontier for $o_i$ (i.e., $\mathcal{G}'(i,s_i^p)$ for all $s_i^p\in\mathcal{S}_i$) is $O(K^2ab\log(Kab))$ and the expected cardinality of $\mathcal{G}'(i,s_i^p)$ is $O(\log(Kab))$.
\end{one step complexity}



\begin{proof}
  According to the assumptions, $\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)\\\otimes \mathcal{G}'(o_{i-1},s_{i-1}^k)\otimes \mathcal{F}(o_i,s_i^p)$ has a cardinality of $ab$ as there is only one tuple in $\mathcal{F}(o_i,s_i^p)$ . $\cup_{s_{i-1}^k \in \mathcal{S}_{i-1} }\{\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)\otimes \mathcal{G}'(o_{i-1},s_{i-1}^k)\otimes \mathcal{F}(o_i,s_i^p)\}$ needs to enumerate all $K$ parallelization configurations of $o_{i-1}$ and thus has a cardinality of $Kab$. According to Lemma~\ref{lemma:frontier complexity} and Lemma~\ref{lemma:random size}, the cost frontier $\mathcal{G}'(o_i, s^p_i)$ has an expected size of $O(\log(Kab))$ and finding it requires a complexity of $O(Kab\log(Kab))$. As all $K$ parallelization configurations of $o_i$ needs to be enumerated to find the collective cost frontier, the overall complexity is $O(K^2ab\log(Kab))$.
\end{proof}


\begin{linear dp complexity}\label{theorem:overall complexity}
For a linear computation graph $\mathcal{G}$ containing $n$ operators, and assume that each operator has at most $K$ parallelization configurations, the overall complexity of Algorithm~\ref{alg:Linear-dp} is $O(n^2K^2\log(K)(\log(n)+\log(K)))$.
\end{linear dp complexity}


\begin{proof}
  For a linear graph $\mathcal{G}'$, the cardinality of $\mathcal{G}'(o_1,s_1^k)$ is 1 for $1 \le k \le K$. The cardinality of $\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)$ is also 1 for any edge $e_{(i-1)i}$, $s_{i-1}^k$ and $s_i^p$. The expected cardinality of $\mathcal{G}'(o_{i-1},s_{i-1}^k)$ is bound by $O(\log(K^{i-2}))$ because there are $K^{i-2}$ partial parallelization strategies from operator $o_1$ to $o_{i-2}$ as each operator has $K$ parallelization configurations. According to Lemma~\ref{theorem:one step complexity}, the complexity for computing the cumulative cost frontier for operator $o_i$ is $O(K^2\log(K^{i-2})\log(K\log(K^{i-2})))$. Summing up the complexity from $o_2$ to $o_n$, we obtain the overall complexity of Algorithm~\ref{alg:Linear-dp} as $\sum_{i=2}^n O(K^2\log(K^{i-2})\log(K\log(K^{i-2})))$, which can be simplified as $O(n^2K^2\log(K)(\log(n)+\log(K)))$.
\end{proof}


For a linear computation graph $\mathcal{G}$, FT-Elimination conducts node elimination (as in Eq.~\ref{equ:node}) to simplify it to a graph that contains only two nodes. In the following, we analyze the complexity of FT-Elimination and compare with FT.

\begin{node elimination complexity}\label{lemma:node elimination complexity}
For node elimination in Eq.~\ref{equ:node}, assume that the operators (i.e., $o_h$, $o_i$ and $o_j$) all have at most $K$ parallelization configurations, $\mathcal{F}(e_{hi}, s_h^w, s_i^k)$ and $\mathcal{F}(e_{ij}, s_i^k, s_j^p)$ have a cardinality of $a$ and $b$, respectively. Then node elimination has a complexity of $O(K^3ab\log(Kab))$.
\end{node elimination complexity}

\begin{proof}
  According to the assumptions, $\cup_{s_i^k\in\mathcal{S}_i}\{\mathcal{F}(e_{hi}, s_h^w, s_i^k) \\ \otimes \mathcal{F}(o_i, s_i^k)\otimes \mathcal{F}(e_{ij}, s_i^k, s_j^p)\}$ has a cardinality of $Kab$ and finding its cost frontier has a complexity of $O(Kab\log(Kab)$ according to Lemma~\ref{lemma:frontier complexity}. For node elimination, we need to enumerate the $K^2$ possible combinations of the possible parallelization configurations of operators $o_h$ and $o_j$ (i.e., $[s_h^w, s_j^p]$). Therefore, the overall complexity of node elimination is $O(K^3ab\log(Kab))$.
\end{proof}

\begin{optcnn complexity}\label{theorem:optcnn complexity}
For a linear computation graph $\mathcal{G}$ containing $n$ operators, and assume that each operator has at most $K$ feasible parallelization configurations, the overall complexity of using FT-Elimination for frontier tracking is $O(n^2K^3\log(K)(\log(n)\\+\log(K)))$.
\end{optcnn complexity}


\begin{proof}
  For a linear graph  $\mathcal{G}'$, both $\mathcal{F}(e_{hi}, s_h^w, s_i^k)$ and $\mathcal{F}(e_{ij}, s_i^k, s_j^p)$ have a cardinality of 1 initially. FT-Elimination will eliminate the nodes in $\mathcal{G}'$ according to the topological order and each time it will eliminate the second node in the remaining graph. For the $i\textsuperscript{th}$ time of node elimination, $\mathcal{F}(e_{hi}, s_h^w, s_i^k)$ has a cardinality of $O(\log(K^{i-1}))$ while the cardinality of  $\mathcal{F}(e_{ij}, s_i^k, s_j^p)$ is 1. According to Lemma~\ref{lemma:node elimination complexity}, the $i\textsuperscript{th}$ node elimination has a complexity of $O(K^3\log(K^{i-1})\log(K\log(K^{i-1})))$. Summing up the complexity from $1$ to $n-2$, the result is $\sum_{i=1}^{n-2} K^3\log(K^{i-1})\log(K\\\log(K^{i-1}))$, which can be reduced to $O(n^2K^3\log(K)(\log(n)+\log(K)))$.
\end{proof}

Combining Theorem~\ref{theorem:overall complexity} and Theorem~\ref{theorem:optcnn complexity}, we can see that LDP reduces the complexity of FT-Elimination by $K$ times when used for frontier tracking. As the number of parallelization configurations for an operator (i.e., $K$) can be large, LDP usually has much shorter running time than FT-Elimination, which we will show in Section~\ref{sec:anylysis}. LDP reduces the complexity because the influence of operator $o_{i-1}$ on the subsequent operators is blocked by the cumulative cost frontier of operator $o_i$ (i.e., $\mathcal{G}'(i,s_i^p)$) and the cardinality of $\mathcal{G}'(i,s_i^p)$ is not large as it is a cost frontier.

%of $\cup_{s_{i-1}^k \in \mathcal{S}_{i-1} }\{\mathcal{F}(e_{(i-1)i},s_{i-1}^k,s_i^p)\otimes \mathcal{G}'(o_{i-1},s_{i-1}^k)\otimes \mathcal{F}(o_i,s_i^p)\}$  

